Determination of droplet size from wide-angle light scattering image data using convolutional neural networks

Wide-angle light scattering (WALS) offers the possibility of a highly temporally and spatially resolved measurement of droplets in spray-based methods for nanoparticle synthesis. The size of these droplets is a critical variable affecting the final properties of synthesized materials such as hetero-aggregates. However, conventional methods for determining droplet sizes from WALS image data are labor-intensive and may introduce biases, particularly when applied to complex systems like spray flame synthesis (SFS). To address these challenges, we introduce a fully automatic machine learning-based approach that employs convolutional neural networks (CNNs) in order to streamline the droplet sizing process. This CNN-based methodology offers further advantages: it requires few manual labels and can utilize transfer learning, making it a promising alternative to conventional methods, specifically with respect to efficiency. To evaluate the performance of our machine learning models, we consider WALS data from an ethanol spray flame process at various heights above the burner surface (HABs), where the models are trained and cross-validated on a large dataset comprising nearly 35000 WALS images.

==> Images/preprocesing.tex <==

\begin{figure}[h]

\centering
\begin{minipage}{0.6\textwidth}
  \centering
  1000x1000\\
  \vspace{5pt}
  \includegraphics[width=\linewidth]{Images/60_01_26_colored_with_colorbar.png}
\end{minipage}
\hspace{40pt}
\begin{minipage}{0.06\textwidth}
  \centering
  56x500\\
  \vspace{5pt}
  \includegraphics[width=\linewidth]{Images/25__colored.png}
\end{minipage}
\caption{A side-by-side comparison of the original  WALS data (left) and the preprocessed image (right). The preprocessing involved applying a polar transform and removing imaging artifacts (bright spots).  The original image has a resolution of $1000\times1000$, while the preprocessed image has a resolution of $56\times496$.}\label{fig:preprocessing}
\end{figure}
